Study of the production of $\Lambda_b^0$ and $\overline{B}^0$ hadrons in $pp$ collisions and first measurement of the $\Lambda_b^0\rightarrow J/\psi pK^-$ branching fraction

The product of the $\Lambda_b^0$ ($\overline{B}^0$) differential production cross-section and the branching fraction of the decay $\Lambda_b^0\rightarrow J/\psi pK^-$ ($\overline{B}^0\rightarrow J/\psi\overline{K}^*(892)^0$) is measured as a function of the beauty hadron transverse momentum, $p_{\rm T}$, and rapidity, $y$. The kinematic region of the measurements is $p_{\rm T}<20~{\rm GeV}/c$ and $2.0<y<4.5$. The measurements use a data sample corresponding to an integrated luminosity of $3~{\rm fb}^{-1}$ collected by the LHCb detector in $pp$ collisions at centre-of-mass energies $\sqrt{s}=7~{\rm TeV}$ in 2011 and $\sqrt{s}=8~{\rm TeV}$ in 2012. Based on previous LHCb results of the fragmentation fraction ratio, $f_{\Lambda_B^0}/f_d$, the branching fraction of the decay $\Lambda_b^0\rightarrow J/\psi pK^-$ is measured to be \begin{equation*} \mathcal{B}(\Lambda_b^0\rightarrow J/\psi pK^-)= (3.17\pm0.04\pm0.07\pm0.34^{+0.45}_{-0.28})\times10^{-4}, \end{equation*} where the first uncertainty is statistical, the second is systematic, the third is due to the uncertainty on the branching fraction of the decay $\overline{B}^0\rightarrow J/\psi\overline{K}^*(892)^0$, and the fourth is due to the knowledge of $f_{\Lambda_b^0}/f_d$. The sum of the asymmetries in the production and decay between $\Lambda_b^0$ and $\overline{\Lambda}_b^0$ is also measured as a function of $p_{\rm T}$ and $y$. The previously published branching fraction of $\Lambda_b^0\rightarrow J/\psi p\pi^-$, relative to that of $\Lambda_b^0\rightarrow J/\psi pK^-$, is updated. The branching fractions of $\Lambda_b^0\rightarrow P_c^+(\rightarrow J/\psi p)K^-$ are determined.

==> figs/8and7ratio/ratio_8_7TeV_B0_pt.tex <==
$\pt [\gevc]$ & \Lb & \Bdb \\
$0<\pt<3$ & $1.11526\pm0.0836815\pm0.0854812$ & $1.1355\pm0.0320715\pm0.0360245$ \\
$3<\pt<4$ & $1.24988\pm0.0958063\pm0.0977816$ & $1.21223\pm0.0443662\pm0.0476986$ \\
$4<\pt<5$ & $1.23381\pm0.085975\pm0.0881154$ & $1.15474\pm0.0345229\pm0.0383433$ \\
$5<\pt<6$ & $1.16141\pm0.0804438\pm0.0824705$ & $1.26325\pm0.0372943\pm0.0415214$ \\
$6<\pt<7$ & $1.22227\pm0.0808773\pm0.0831072$ & $1.193\pm0.0350726\pm0.0390797$ \\
$7<\pt<8$ & $1.26305\pm0.0866346\pm0.0888597$ & $1.15838\pm0.036623\pm0.0402665$ \\
$8<\pt<9$ & $1.27381\pm0.0949315\pm0.0970008$ & $1.22906\pm0.0407551\pm0.0444562$ \\
$9<\pt<10$ & $1.14269\pm0.0914804\pm0.093211$ & $1.24109\pm0.0433535\pm0.0469159$ \\
$10<\pt<12$ & $1.40171\pm0.0996938\pm0.102077$ & $1.20471\pm0.0336611\pm0.0378955$ \\
$12<\pt<20$ & $1.20199\pm0.0738167\pm0.0761745$ & $1.34095\pm0.0326575\pm0.0379725$ \\


==> figs/8and7ratio/ratio_8_7TeV_B0_y.tex <==
$\y$ & \Lb & \Bdb \\
$2<y<2.5$ & $1.33865\pm0.0516341\pm0.055138$ 
$2.5<y<3$ & $1.16612\pm0.0196939\pm0.0259181$ 
$3<y<3.5$ & $1.10091\pm0.0152885\pm0.022063$ 
$3.5<y<4$ & $1.14863\pm0.0207446\pm0.0265667$ 
$4<y<4.5$ & $1.10692\pm0.0413974\pm0.0443796$ 

$2<y<2.5$ & $1.3156\pm0.12078\pm0.122521$ 
$2.5<y<3$ & $1.2881\pm0.0607839\pm0.0640376$ 
$3<y<3.5$ & $1.12266\pm0.0509064\pm0.0538513$ 
$3.5<y<4$ & $1.08467\pm0.0666576\pm0.0687838$ 
$4<y<4.5$ & $1.00072\pm0.140257\pm0.141128$ 


==> table/RLbBdb/ans.tex <==
 &	 $2<y<2.5$ &	 $2.5<y<3$ &	 $3<y<3.5$ &	 $3.5<y<4$ &	 $4<y<4.5$ &	\\ 
	2011 &	 $0.108 \pm 0.0079 \pm 0.0031$ &	 $0.111 \pm 0.0037 \pm 0.0022$ &	 $0.115 \pm 0.0035 \pm 0.0022$ &	 $0.118 \pm 0.0047 \pm 0.0028$ &	 $0.117 \pm 0.012 \pm 0.0055$ &	\\ 
	2012 &	 $0.106 \pm 0.0062 \pm 0.0029$ &	 $0.123 \pm 0.0035 \pm 0.0029$ &	 $0.118 \pm 0.0033 \pm 0.0028$ &	 $0.111 \pm 0.0042 \pm 0.0034$ &	 $0.106 \pm 0.0093 \pm 0.0038$ &	\\ 
	

==> table/RLbBdb/ans_11.tex <==
\RLbBdb     & 2011                                       & 2012 \\
$0<\pt<1$   & \multirow{3}{*}{$0.122\pm0.0048\pm0.0058$} & 
$1<\pt<2$   &                            & 
$2<\pt<3$   &                            & 
$3<\pt<4$   & $0.118\pm0.0047\pm0.0056$  & 
$4<\pt<5$   & $0.116\pm0.0044\pm0.0049$  & 
$5<\pt<6$   & $0.122\pm0.0046\pm0.0055$  & 
$6<\pt<7$   & $0.107\pm0.0041\pm0.0044$  & 
$7<\pt<8$   & $0.0985\pm0.0040\pm0.0042$ & 
$8<\pt<9$   & $0.0935\pm0.0042\pm0.0040$ & 
$9<\pt<10$  & $0.1010\pm0.0049\pm0.0046$ & 
$10<\pt<12$ & $0.0785\pm0.0033\pm0.0032$ & 
$12<\pt<20$ & $0.0732\pm0.0028\pm0.0026$ & 
	
 & $0<\pt<1$ 	 & $1<\pt<2$ 	 & $2<\pt<3$ 	 & $3<\pt<4$ 	\\ 
	Ratio &	 $0.12 \pm 0.0097 \pm 0.015$ 	&	 $0.124 \pm 0.0058 \pm 0.0092$ 	&	 $0.117 \pm 0.004 \pm 0.0079$ 	&	 $0.122 \pm 0.0033 \pm 0.0067$ 	\\ 
	 & $4<\pt<5$ 	 & $5<\pt<6$ 	 & $6<\pt<7$ 	 & $7<\pt<8$ 	\\ 
	Ratio &	 $0.124 \pm 0.003 \pm 0.0059$ 	&	 $0.112 \pm 0.0027 \pm 0.005$ 	&	 $0.109 \pm 0.0027 \pm 0.0047$ 	&	 $0.107 \pm 0.0028 \pm 0.0047$ 	\\ 
	 & $8<\pt<9$ 	 & $9<\pt<10$ 	 & $10<\pt<12$ 	 & $12<\pt<20$ 	\\ 
	Ratio &	 $0.0969 \pm 0.0028 \pm 0.0047$ 	&	 $0.093 \pm 0.0031 \pm 0.0046$ 	&	 $0.0914 \pm 0.0026 \pm 0.0041$ 	&	 $0.0656 \pm 0.0016 \pm 0.0024$ 	\\ 
	

==> table/RLbBdb/ans_12.tex <==
 & $0<\pt<1$ 	 & $1<\pt<2$ 	 & $2<\pt<3$ 	 & $3<\pt<4$ 	\\ 
	Ratio &	 $0.12 \pm 0.0097 \pm 0.015$ 	&	 $0.124 \pm 0.0058 \pm 0.0092$ 	&	 $0.117 \pm 0.004 \pm 0.0079$ 	&	 $0.122 \pm 0.0033 \pm 0.0067$ 	\\ 
	 & $4<\pt<5$ 	 & $5<\pt<6$ 	 & $6<\pt<7$ 	 & $7<\pt<8$ 	\\ 
	Ratio &	 $0.124 \pm 0.003 \pm 0.0059$ 	&	 $0.112 \pm 0.0027 \pm 0.005$ 	&	 $0.109 \pm 0.0027 \pm 0.0047$ 	&	 $0.107 \pm 0.0028 \pm 0.0047$ 	\\ 
	 & $8<\pt<9$ 	 & $9<\pt<10$ 	 & $10<\pt<12$ 	 & $12<\pt<20$ 	\\ 
	Ratio &	 $0.0969 \pm 0.0028 \pm 0.0047$ 	&	 $0.093 \pm 0.0031 \pm 0.0046$ 	&	 $0.0914 \pm 0.0026 \pm 0.0041$ 	&	 $0.0656 \pm 0.0016 \pm 0.0024$ 	\\ 
	

==> table/RLbBdb/ans_pt.tex <==
\pt [\gevc]     & 2011                                       & 2012 \\
\hline
$0<\pt<1$   & \multirow{3}{*}{$0.1220\pm0.0048\pm0.0058$} & $0.120\xx\pm0.010\xx\pm0.015\xx$ \\
$1<\pt<2$   &                            & $0.1240\pm0.0058\pm0.0092$ \\
$2<\pt<3$   &                            & $0.1170\pm0.0040\pm0.0079$ \\ 
$3<\pt<4$   & $0.1180\pm0.0047\pm0.0056$ & $0.1220\pm0.0033\pm0.0067$ \\ 
$4<\pt<5$   & $0.1160\pm0.0044\pm0.0049$ & $0.1240\pm0.0030\pm0.0059$ \\ 
$5<\pt<6$   & $0.1220\pm0.0046\pm0.0055$ & $0.1120\pm0.0027\pm0.0050$ \\
$6<\pt<7$   & $0.1070\pm0.0041\pm0.0044$ & $0.1090\pm0.0027\pm0.0047$ \\ 
$7<\pt<8$   & $0.0985\pm0.0040\pm0.0042$ & $0.1070\pm0.0028\pm0.0047$ \\ 
$8<\pt<9$   & $0.0935\pm0.0042\pm0.0040$ & $0.0969\pm0.0028\pm0.0047$ \\
$9<\pt<10$  & $0.1010\pm0.0049\pm0.0046$ & $0.0930\pm0.0031\pm0.0046$ \\
$10<\pt<12$ & $0.0785\pm0.0033\pm0.0032$ & $0.0914\pm0.0026\pm0.0041$ \\ 
$12<\pt<20$ & $0.0732\pm0.0028\pm0.0026$ & $0.0656\pm0.0016\pm0.0024$ \\ 
	
	


==> table/RLbBdb/ans_y.tex <==
            & 2011                       & 2012 \\
\hline
$2.0<y<2.5$ & $0.1080\pm0.0079\pm0.0031$ & $0.1060\pm0.0062\pm0.0029$ \\
$2.5<y<3.0$ & $0.1110\pm0.0037\pm0.0022$ & $0.1230\pm0.0035\pm0.0029$ \\
$3.0<y<3.5$ & $0.1150\pm0.0035\pm0.0022$ & $0.1180\pm0.0033\pm0.0028$ \\
$3.5<y<4.0$ & $0.1180\pm0.0047\pm0.0028$ & $0.1110\pm0.0042\pm0.0034$ \\
$4.0<y<4.5$ & $0.1170\pm0.0120\pm0.0055$ & $0.1060\pm0.0093\pm0.0038$ \\ 


==> table/X1D/ans_pt_11.tex <==
 $\pt[\gevc]$ & 2011 $\Lb$                    & 2011 $\Bdb$ \\
\hline
 $0<\pt<3$    & $0.743\pm0.028\pm0.041$       & $6.07\pm0.07\pm0.24$ \\
 $3<\pt<4$    & $1.020\pm0.038\pm0.055$       & $8.66\pm0.13\pm0.36$ \\
 $4<\pt<5$    & $0.839\pm0.030\pm0.043$       & $7.24\pm0.09\pm0.29$ \\
 $5<\pt<6$    & $0.661\pm0.024\pm0.035$       & $5.42\pm0.07\pm0.22$ \\ 
 $6<\pt<7$    & $0.432\pm0.015\pm0.022$       & $4.05\pm0.05\pm0.17$ \\
 $7<\pt<8$    & $0.307\pm0.012\pm0.015$       & $3.11\pm0.04\pm0.13$ \\
 $8<\pt<9$    & $0.202\pm0.009\pm0.010$       & $2.16\pm0.031\pm0.091$ \\
 $9<\pt<10$   & $0.1510\pm0.0070\pm0.0079$    & $1.490\pm0.023\pm0.063$ \\ 
 $10<\pt<12$  & $0.0743\pm0.0030\pm0.0037$    & $0.946\pm0.012\pm0.038$ \\
 $12<\pt<20$  & $0.01880\pm0.00069\pm0.00087$ & $0.257\pm0.003\pm0.010$ \\ 



==> table/X1D/ans_pt_12.tex <==
 \pt [\gevc] & 2012 \Lb & 2012 \Bdb \\
\hline
 $0<\pt<1$   & $0.331\pm0.025\pm0.040$     & $\xx2.76\pm0.07\pm0.15$ \\
 $1<\pt<2$   & $0.925\pm0.041\pm0.070$     & $\xx7.45\pm0.10\pm0.32$ \\
 $2<\pt<3$   & $1.230\pm0.039\pm0.084$     & $10.50\pm0.13\pm0.47$ \\
 $3<\pt<4$   & $1.280\pm0.032\pm0.074$     & $10.50\pm0.11\pm0.44$ \\
 $4<\pt<5$   & $1.040\pm0.024\pm0.055$     & $\xx8.37\pm0.07\pm 0.33$ \\
 $5<\pt<6$   & $0.767\pm0.017\pm0.039$     & $\xx6.85\pm0.06\pm0.27$ \\
 $6<\pt<7$   & $0.528\pm0.012\pm0.026$     & $\xx4.83\pm0.04\pm0.19$ \\
 $7<\pt<8$   & $0.387\pm0.009\pm0.019$     & $\xx3.61\pm0.03\pm 0.14$ \\ 
 $8<\pt<9$   & $0.258\pm0.007\pm0.014$	   & $\xx2.66\pm0.03\pm0.11$ \\
 $9<\pt<10$  & $0.1730\pm0.0054\pm0.0093$  & $1.860\pm0.019\pm0.075$ \\
 $10<\pt<12$ & $0.1040\pm0.0028\pm0.0053$  & $1.140\pm0.009\pm0.044$ \\
 $12<\pt<20$ & $0.0226\pm0.00053\pm0.0010$ & $0.344\pm0.002\pm0.013$ \\ 


==> table/X1D/ans_y.tex <==
             & 2011 \Lb             & 2012 \Lb            \\
\hline
$2.0<y<2.5$ & $2.95\pm0.15\pm0.18$ & $3.88\pm0.11\pm0.23$ \\
$2.5<y<3.0$ & $3.01\pm0.07\pm0.13$ & $3.87\pm0.06\pm0.17$ \\
$3.0<y<3.5$ & $2.78\pm0.05\pm0.12$ & $3.12\pm0.04\pm0.14$ \\
$3.5<y<4.0$ & $2.14\pm0.05\pm0.10$ & $2.32\pm0.04\pm0.12$ \\
$4.0<y<4.5$ & $1.42\pm0.09\pm0.13$ & $1.42\pm0.07\pm0.12$ \\
\hline
            & 2011 \Bdb            & 2012 \Bdb  \\
\hline
$2.0<y<2.5$ & $27.3\pm0.5\pm1.2$     & $36.5\pm0.4\pm1.5$ \\
$2.5<y<3.0$ & $27.0\pm0.2\pm1.0$     & $31.5\pm0.2\pm1.1$ \\
$3.0<y<3.5$ & $24.10\pm0.14\pm0.90$  & $26.50\pm0.11\pm0.94$ \\
$3.5<y<4.0$ & $18.10\pm0.13\pm 0.69$ & $20.80\pm0.11\pm0.76$ \\
$4.0<y<4.5$ & $12.10\pm0.19\pm0.52$  & $13.40\pm0.15\pm0.56$ \\ 


==> table/number/integral/B011/ans_REF.tex <==
41.37\pm0.23\stat\pm1.58\syst\pm4.47(\BR)\mub

